PentestGPT: An LLM-empowered Automatic Penetration Testing Tool

Penetration testing, a crucial industrial practice for ensuring system security, has traditionally resisted automation due to the extensive expertise required by human professionals. Large Language Models (LLMs) have shown significant advancements in various domains, and their emergent abilities suggest their potential to revolutionize industries. In this research, we evaluate the performance of LLMs on real-world penetration testing tasks using a robust benchmark created from test machines with platforms. Our findings reveal that while LLMs demonstrate proficiency in specific sub-tasks within the penetration testing process, such as using testing tools, interpreting outputs, and proposing subsequent actions, they also encounter difficulties maintaining an integrated understanding of the overall testing scenario. In response to these insights, we introduce PentestGPT, an LLM-empowered automatic penetration testing tool that leverages the abundant domain knowledge inherent in LLMs. PentestGPT is meticulously designed with three self-interacting modules, each addressing individual sub-tasks of penetration testing, to mitigate the challenges related to context loss. Our evaluation shows that PentestGPT not only outperforms LLMs with a task-completion increase of 228.6\% compared to the \gptthree model among the benchmark targets but also proves effective in tackling real-world penetration testing challenges. Having been open-sourced on GitHub, PentestGPT has garnered over 4,700 stars and fostered active community engagement, attesting to its value and impact in both the academic and industrial spheres.

==> Tex/Revision.tex <==
\clearpage
\section*{Revision Summary}


We extend our deepest gratitude to the reviewers for their insightful comments and constructive feedback. Following the revision plan previously outlined, we have diligently updated our manuscript. This update includes additional experiments that provide a more accurate evaluation of Excalibur's performance. Notably, we have expanded our testing to encompass Excalibur’s involvement in open-source CTF challenges, where it achieved competitive results. We have attached the revised version of the manuscript for your review, where all the changes are highlighted in red color.


Below, we summarize the key changes made. We kindly request that you review the manuscript and inform us of any further modifications that may be required.



\vspace{1mm}\noindent\textbf{1. Benchmark Construction}

\vspace{1mm}\noindent We have thoroughly revised Section~\ref{sec:benchmark} \textit{Penetration-Testing Benchmark} to enhance clarity around the benchmark creation and validation processes. We now provide detailed explanations of how the benchmark machines were selected from open-source penetration testing targets, and describe how certified penetration testers were instructed to conduct evaluations in both terminal and GUI settings. Notably, we now include detailed backgrounds and expertise of the human testers to emphasize the robustness of our study (Page-6). Additionally, we discuss our plans for integrating large vision language models (LVLM) to automate and refine the testing process in future work.


\vspace{1mm}\noindent\textbf{2. Benchmark Evaluation}

\vspace{1mm}\noindent We have updated Section-4-Exploratory-Study to ensure a fair and consistent evaluation framework. Details about the evaluation setups have been expanded, and experiments were aligned with later sections using the GPT-4-32k model. The revised results are presented in Table~\ref{tab:overall-performance} (Page-7). While GPT-4-32k shows improved performance over GPT-3.5 and Bard in penetration testing tasks, it still exhibits issues with context retention and task-focus as discussed in Section~\ref{sec:comparative-analysis} Comparative-Analysis. Our overall conclusions, such as LLMs struggle to maintain long-term memory and they over-focus on recent tasks, remain unchanged.

\vspace{1mm}\noindent\textbf{3. Penetration Testing Tree Presentation and Usage}

\vspace{1mm}\noindent In Section~\ref{sec:reasoning-module}-Reasoning-Module, we have refined the presentation of the Penetration Testing Tree (PTT). As suggested, a complete example of a PTT is now included in the Appendix, demonstrating the process using *Hackable-II*, a target from our open-source penetration testing benchmark. We hope this help to clarify how our solution works from an overview perspective.

\vspace{1mm}\noindent\textbf{4. Experiments on Open-source Targets}

\vspace{1mm}\noindent Following your recommendation, we have broadened our evaluation by participating in the open-source CTF challenge, PicoCTF, hosted by Carnegie Mellon University and redpwn. This competition's challenges are freely available online, providing transparent and accessible data on our tool's performance. Employing the same experimental setup used with \tool{}-GPT4-32k five attempts per target, our solution accumulated 1400 points, ranking 24th out of 248 teams with valid submissions. This performance provides a clear, empirical demonstration of our tool's capabilities in a competitive and realistic environment.



\vspace{1mm}\noindent\textbf{5. Improve Evaluation}

\vspace{1mm}\noindent In response to feedback, we have included the average performance of Excalibur across benchmarks, with the updated results displayed in Table~\ref{tab:htb-challenges} (Page 14). We also report the average performance of the extended experiments on the open-source CTF challenges in Table~\ref{tab:picomini-challenges} in Appendix.



\vspace{1mm}\noindent\textbf{6. Discussion on Underperformance Cases}

\vspace{1mm}\noindent We have elaborated on the reasons behind the underperformance of our tool in high-level penetration testing challenges and discussed potential strategies for improvement (Section~\ref{sec:evaluation:strategy-evaluation}, Page 13). Furthermore, we have added a thorough discussion on the ethical implications of our research in Section~\ref{sec:discussion}-Discussion (page 15).



